Conditional Reconstruction for Open-set Semantic Segmentation

Open set segmentation is a relatively new and unexploredtask, with just a handful of methods proposed to model suchtasks.We propose a novel method called CoReSeg thattackles the issue using class conditional reconstruction ofthe input images according to their pixelwise mask. Ourmethod conditions each input pixel to all known classes,expecting higher errors for pixels of unknown classes. Itwas observed that the proposed method produces better se-mantic consistency in its predictions, resulting in cleanersegmentation maps that better fit object boundaries. CoRe-Seg outperforms state-of-the-art methods on the Vaihin-gen and Potsdam ISPRS datasets, while also being com-petitive on the Houston 2018 IEEE GRSS Data Fusiondataset. Official implementation for CoReSeg is availableat:https://github.com/iannunes/CoReSeg.

==> sec_old_intro.tex <==
% \section{Introduction}
% \label{sec:intro}

% In recent years, computer vision research has significantly improved many aspects of visual recognition and achieved human-level performance for countless tasks. Despite the many advances, there are still difficult challenges when facing real-world problems. A major not yet solved challenge is related to the incomplete knowledge of the world during training or the existence of unknown samples during inference. So-called Open-Set Recognition (OSR) tasks have caught the interest of the research community with multiple recently proposed methods for classification problems \cite{bendale2016,sun2020,oza_patel_2019,cui2020,guo2021}. However, very few works have dealt with different visual tasks, such as segmentation or object detection.

% \renewcommand{\currprop}{0.85\columnwidth}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\currprop]{figs/OpenSet_Intro.pdf}
%     \caption{Open set segmentation problem: input image labels contain samples of 4 KKCs: Impervious Surfaces, Building, Low Vegetation and High Vegetation for training, as we can see in the image, not all pixels are labeled correctly, some areas contain cars labeled as Impervious Surfaces. The purpose of open set segmentation is to recognize pixels of unknown classes during testing.}
%     \label{fig:intro}
% \end{figure}

% Open-Set Semantic Segmentation (O3S) refers to the set of algorithms that address the problem of identifying pixels of unknown 
% %(out-of-distribution) 
% classes at inference time, while still correctly classifying pixels of the known classes learned in training \cite{oliveira2021}. O3S is an inherently harder problem due to its dense labeling nature when compared to Open-Set classification. This explains why there is still a gap in the literature with only a handful of works tackling the issue \cite{cui2020}.

% %The remaining of this work is organized as follows: Section~\ref{sec:related} discuss some of the most important previous works in Open-Set semantic segmentation; Section~\ref{sec:method} introduces the proposed methods; Section~\ref{sec:setup} briefly explains the experimental setup and describes the datasets used; Section~\ref{sec:results} presents a discussion of the results; finally, Section~\ref{sec:conclusion} concludes the paper and presents possible future works.
% %To the best of our knowledge, only a few works in the literature tackle the O3S problem.
% In 2016, Bendale \textit{et al.} \cite{bendale2016} proposed OpenMax to identify out-of-distribution (OOD) whole images. Silva \textit{et al.} \cite{silva2020} later proposed OpenPixel based on OpenMax, using the existing framework for patchwise O3S. OpenPixel has a major drawback of being extremely inefficient during both training and testing, however.
% %\cite{silva2020} later proposed the OpenPixel method on top of OpenMax and based on patchwise training of a specifically designed CNN for image classification by \cite{nogueira2016}, as a patchwise model, OpenPixel is higly inefficient both for training and testing.
% %Cui \textit{et al.} \cite{cui2020} proposed a method that employs a non-parametric statistical Mann-Whitney U test on a Closed-Set segmentation output to determine the existence of unknown classes. In the predicted unknown areas, the distribution of the uncertainties is approximated as a histogram and the local minimum determines a threshold that defines which pixels are set as unknown. This adaptive method is applicable to each image independently.
% A non-parametric statistical adaptive OS3 method was proposed by \cite{cui2020}, it uses the Mann-Whitney U test on a Closed-Set segmentation output to determine the existence of unknown classes in each image and uses an adaptive threshold that defines which pixels are set as unknown.

% The first fully convolutional architectures for O3S were proposed by Oliveira \textit{et al.} \cite{oliveira2021}. Open Fully Convolutional Network (OpenFCN) is a fully convolutional extension of OpenPixel \cite{silva2020} for dense labeling tasks. Open Principal Component Scoring (OpenPCS) \cite{oliveira2021} uses the intermediate feature activations from deep Closed-Set networks to fit Gaussian distributions in a low-dimensional projection, obtaining a data likelihood score pointing to OOD pixelwise detection.
% \jef{Quais são as limitações dos métodos existentes que justificam a criação de um outro?
% Como o método proposto se compara com a literatura do ponto de vista conceitual? 
% O que o método CoReSeg tras de novidade?
% Precisamos melhorar essa discussão e a venda do artigo, no geral.}

% In this work, we focus on exploring solutions for O3S by proposing a new end-to-end fully convolutional method referred to as Conditional Reconstruction for Open-Set Segmentation (\methodname), capable of achieving state-of-the-art results in at least two datasets available in the literature. 
% \jef{O que é reconstrução condicional? Isso precisa ser respondido aqui ou na Sec. 2.}
% The current work includes the following contributions: (i) a new method for O3S called \methodname; (ii) state-of-the-art O3S results for two remote sensing segmentation datasets.; (iii) pixelwise dimensionality-aware conditioning technique.

==> sec_old_related.tex <==
% \section{Related work}
% \label{sec:related}

% To the best of our knowledge, only a few works in the literature tackle the OSS problem. In 2016, Bendale \textit{et al.} \cite{bendale2016} proposed OpenMax to identify out-of-distribution (OOD) whole images. Silva \textit{et al.} \cite{silva2020} later proposed OpenPixel based on OpenMax, using the existing framework for patchwise OSS. OpenPixel has a major drawback of being extremely inefficient during both training and testing, however.
% %\cite{silva2020} later proposed the OpenPixel method on top of OpenMax and based on patchwise training of a specifically designed CNN for image classification by \cite{nogueira2016}, as a patchwise model, OpenPixel is higly inefficient both for training and testing.

% %Cui \textit{et al.} \cite{cui2020} proposed a method that employs a non-parametric statistical Mann-Whitney U test on a Closed-Set segmentation output to determine the existence of unknown classes. In the predicted unknown areas, the distribution of the uncertainties is approximated as a histogram and the local minimum determines a threshold that defines which pixels are set as unknown. This adaptive method is applicable to each image independently.

% A non-parametric statistical adaptive OSS method was proposed by \cite{cui2020}, it uses the Mann-Whitney U test on a Closed-Set segmentation output to determine the existence of unknown classes in each image and uses an adaptive threshold that defines which pixels are set as unknown.

% The first fully convolutional architectures for OSS were proposed by Oliveira \textit{et al.} \cite{oliveira2021}. Open Fully Convolutional Network (OpenFCN) is a fully convolutional extension of OpenPixel \cite{silva2020} for dense labeling tasks. Open Principal Component Scoring (OpenPCS) \cite{oliveira2021} uses the intermediate feature activations from deep Closed-Set networks to fit Gaussian distributions in a low-dimensional projection, obtaining a data likelihood score pointing to OOD pixelwise detection.

% %\subsection{Conditioning}
% %\label{ssec:Conditioning}

% %Feature-wise Linear Modulation (FiLM) by \cite{perez_strub_de-vries_dumoulin_courville_2018} condition a network through affine transformations, and can be formalized as: \(\ FiLM(x) = \gamma(z) · x + \beta(z)\), where x is the input of the FiLM layer, and \(\gamma\) and \(\beta\) are learnable parameters. 

==> tab_potsdam.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{0.7}% Tighter
    \begin{tabular}{@{}ccccccc@{}}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{5}{c}{\textbf{UUCs}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{OA}}} \\ \cmidrule(lr){2-6}
        \multicolumn{1}{c}{} & \multicolumn{1}{l}{\textit{\textbf{0}}} & \multicolumn{1}{l}{\textit{\textbf{1}}} & \multicolumn{1}{l}{\textit{\textbf{2}}} & \multicolumn{1}{l}{\textit{\textbf{3}}} & \multicolumn{1}{l}{\textit{\textbf{4}}} & \multicolumn{1}{c}{} \\ \midrule
        Softmax(1) & 0.66 & 0.49 & 0.53 & 0.64 & 0.76 & 0.62 \\ 
        Softmax(2) & 0.68 & 0.53 & 0.60 & 0.62 & 0.66 & 0.62 \\ 
        Softmax(3) & 0.75 & 0.50 & 0.74 & \textbf{0.65} & 0.68 & 0.66 \\ 
        OpenPCS(1) & 0.83 & 0.87 & 0.28 & 0.54 & 0.77 & 0.66 \\ 
        OpenPCS(2) & 0.66 & 0.86 & 0.71 & 0.57 & 0.86 & 0.73 \\
        OpenPCS(3) & \textbf{0.88} & 0.86 & 0.42 & 0.53 & 0.84 & 0.70 \\ 
        OpenIPCS(1) & 0.84 & 0.88 & 0.41 & 0.54 & \textbf{0.91} & 0.72 \\ 
        OpenIPCS(2) & 0.64 & 0.86 & \textbf{0.76} & 0.55 & 0.83 & 0.73 \\ 
        \methodname(3) & 0.82 & \textbf{0.90} & 0.70 & 0.63 & 0.77 & \textbf{0.76} \\ \bottomrule
    \end{tabular}
    \caption{AUROC results for the Potsdam dataset.}
    \label{tab:potsdam results}
\end{table}
